Autoinverse: Uncertainty Aware Inversion of Neural Networks

Neural networks are powerful surrogates for numerous forward processes. The inversion of such surrogates is extremely valuable in science and engineering. The most important property of a successful neural inverse method is the performance of its solutions when deployed in the real world, i.e., on the native forward process (and not only the learned surrogate). We propose Autoinverse, a highly automated approach for inverting neural network surrogates. Our main insight is to seek inverse solutions in the vicinity of reliable data which have been sampled form the forward process and used for training the surrogate model. Autoinverse finds such solutions by taking into account the predictive uncertainty of the surrogate and minimizing it during the inversion. Apart from high accuracy, Autoinverse enforces the feasibility of solutions, comes with embedded regularization, and is initialization free. We verify our proposed method through addressing a set of real-world problems in control, fabrication, and design.

==> sections/Experiments.tex <==
\section{Experiments}
\label{Experiments}
\subsection{1-D Toy}
\label{1-D_Toy}
In this experiment, we used synthetic toy data with known amount of noise and sparsity, to evaluate the performance of our method.
%
The function is a simple sine wave that is augmented with Gaussian noise in some regions.
%
Moreover in some regions, the dataset is sampled sparsely thus leads to high epistemic uncertainty.
%
%
\subsection{2-D Toy}
\label{2-D_Toy}
2-D toy example is a function that maps any point on $(x,y)$ plane to performances $(f_{1},f_{2})$, where $f_{1} = 2\times x$ and $f_{2} =  x^2 + y^2$.
%
The performance space in some regions is augmented with Gaussian noise. 
%
\subsection{halftone Experiment}
\label{halftone}
(To be edited) Almost all printers are binary devices: they either print at a given location or leave it unprinted. 
% 
For printing images with a continuous tone impression, {halftoning} algorithms take advantage of the low-pass filtering property of the human visual system \cite{kang92}. 
%
Halftoning methods create spatial binary patterns of dots with different sizes and spacings so that, when viewed from a sufficient distance, give the impression of continuous tone with the least objectionable artifacts. 
%
In most color halftoning methods, a halftone layer is created for each ink separately and the final color-halftone image is formed by the superposition of all layers. 
% 
\begin{figure}[t] \label{fig:demichel}
\centering
\includegraphics[width = 0.7\linewidth]{figs/DeMichel_random_decomposed.pdf}
\caption{A halftone patch made of three inks.}
\label{fig:demichel}
\end{figure}
%
Here in this experiment we use a neural network to predict the colorometric values from the mixture of area coverage.
%
We train the network on a dataset that comprise of halftone patterns of an 8-ink printer and (A*,B*) values of the resulting colors for around 34,000 combinations.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
